A quantum walk control plane for distributed quantum computing in quantum networks

Quantum networks are complex systems formed by the interaction among quantum processors through quantum channels. Analogous to classical computer networks, quantum networks allow for the distribution of quantum computation among quantum computers. In this work, we describe a quantum walk protocol to perform distributed quantum computing in a quantum network. The protocol uses a quantum walk as a quantum control signal to perform distributed quantum operations. We consider a generalization of the discrete-time coined quantum walk model that accounts for the interaction between a quantum walker system in the network graph with quantum registers inside the network nodes. The protocol logically captures distributed quantum computing, abstracting hardware implementation and the transmission of quantum information through channels. Control signal transmission is mapped to the propagation of the walker system across the network, while interactions between the control layer and the quantum registers are embedded into the application of coin operators. We demonstrate how to use the quantum walker system to perform a distributed CNOT operation, which shows the universality of the protocol for distributed quantum computing. Furthermore, we apply the protocol to the task of entanglement distribution in a quantum network.

==> drawings/k2/k2.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$0$};
    \node[state] (1) [right of = 0] {$1$};
    \path[->] 
        (0) edge [loop above] node {$\ket{10}$} ()
        (0) edge [bend left] node {$\ket{01}$} (1)
        (1) edge [bend left] node {$\ket{00}$} (0)
        (1) edge [loop above] node {$\ket{11}$} ();
\end{tikzpicture}

==> drawings/k2/k2_coin.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$0$};
    \node[state] (1) [right of = 0] {$1$};
    \path[->] 
        (0) edge [bend left] node {$\ket{01}$} (1)
        (1) edge [loop above] node {$\ket{11}$} ();
\end{tikzpicture}

==> drawings/k2/k2_entangled.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$0$};
    \node[state] (1) [right of = 0] {$1$};
    \path[->] 
        % (0) edge [loop above] node {$\ket{10}$} ()
        % (0) edge [bend left] node {$\ket{01}$} (1)
        (1) edge [bend left] node {$\ket{00}$} (0)
        (1) edge [loop above] node {$\ket{11}$} ();
\end{tikzpicture}

==> drawings/k2/k2_separable.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$0$};
    \node[state] (1) [right of = 0] {$1$};
    \path[->] 
        (0) edge [loop above] node {$\ket{10}$} ()
        (1) edge [bend left] node {$\ket{00}$} (0);
\end{tikzpicture}

==> drawings/k4/k4.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$00$};
    \node[state] (1) [right of = 0] {$01$};
    \node[state] (2) [below of = 0] {$10$};
    \node[state] (3) [below of = 1] {$11$};
    \path[-] 
        (0) edge [loop above] node {} ()
        (1) edge [loop above] node {} ()
        (2) edge [loop below] node {} ()
        (3) edge [loop below] node {} ()
        (0) edge [] node {} (1)
        % (1) edge [bend left] node {$\ket{11}$} (0)
        (0) edge [] node {} (2)
        % (2) edge [bend left] node {$\ket{11}$} (0)
        (0) edge [] node {} (3)
        % (3) edge [] node {$\ket{1111}$} (0)
        (1) edge [] node {} (2)
        % (2) edge [bend left] node {$\ket{11}$} (1)
        (1) edge [] node {} (3)
        % (3) edge [] node {$\ket{0011}$} (1)
        (2) edge [] node {} (3);
        % (3) edge [] node {$\ket{1100}$} (2);
\end{tikzpicture}


==> drawings/k4/k4_c1.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$00$};
    \node[state] (1) [right of = 0] {$01$};
    \node[state] (2) [below of = 0] {$10$};
    \node[state] (3) [below of = 1] {$11$};
    \path[->] 
        % (3) edge [loop below] node {$\ket{1111}$} ()
        (3) edge [] node {$\ket{0000}$} (0);
        % (3) edge [] node {$\ket{0011}$} (1)
        % (3) edge [] node {$\ket{1100}$} (2);
\end{tikzpicture}

==> drawings/k4/k4_c2.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$00$};
    \node[state] (1) [right of = 0] {$01$};
    \node[state] (2) [below of = 0] {$10$};
    \node[state] (3) [below of = 1] {$11$};
    \path[->] 
        (3) edge [loop below] node {$\ket{1111}$} ()
        (3) edge [] node {$\ket{0000}$} (0);
        % (3) edge [] node {$\ket{0011}$} (1)
        % (3) edge [] node {$\ket{1100}$} (2);
\end{tikzpicture}

==> drawings/k4/k4_ent.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$00$};
    \node[state] (1) [right of = 0] {$01$};
    \node[state] (2) [below of = 0] {$10$};
    \node[state] (3) [below of = 1] {$11$};
    \path[->] 
        (3) edge [loop below] node {$\ket{1111}$} ()
        (3) edge [] node {$\ket{0000}$} (0)
        (3) edge [] node {$\ket{0011}$} (1)
        (3) edge [] node {$\ket{1100}$} (2);
\end{tikzpicture}

==> drawings/k4/k4_sep.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$00$};
    \node[state] (1) [right of = 0] {$01$};
    \node[state] (2) [below of = 0] {$10$};
    \node[state] (3) [below of = 1] {$11$};
    \path[->] 
        (0) edge [loop above] node {$\ket{1010}$} ()
        (1) edge [] node {$\ket{1000}$} (0)
        (2) edge [] node {$\ket{0010}$} (0)
        (3) edge [] node {$\ket{0000}$} (0);
\end{tikzpicture}

==> drawings/swapping/chain.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$A$};
    \node[state] (1) [right of = 0] {$u$};
    \node[state] (2) [right of = 1] {$B$};
    \path[-] 
        (0) edge node {} (1)
        (1) edge node {} (2);
\end{tikzpicture}

==> drawings/swapping/coin1.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$00$};
    \node[state] (1) [right of = 0] {$01$};
    \node[state] (2) [below of = 0] {$10$};
    \node[state] (3) [below of = 1] {$11$};
    \path[->] 
        (3) edge [loop below] node {$\ket{1111}$} ()
        (3) edge [] node {$\ket{0000}$} (0)
        (3) edge [] node {$\ket{0011}$} (1)
        (3) edge [] node {$\ket{1100}$} (2);
\end{tikzpicture}

==> drawings/swapping/star.tex <==
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
    \node[state] (0) {$A$};
    \node[state] (1) [right of = 0] {$u$};
    \node[state] (2) [right of = 1] {$B$};
    \node[state] (3) [above of = 1] {$C$};
    \path[-] 
        (0) edge node {} (1)
        (1) edge node {} (2)
        (1) edge node {} (3);
\end{tikzpicture}

==> state_qwalk.tex <==
\section{Walkers that carry state}

The overall takeaway from Section \ref{sec:assisted} is that coupling the qubits of a network with a quantum walker system is enough to route entanglement. Nonetheless, the generation of a maximally entangled state is dependent on a uniform superposition of vertices. A different formulation that allows for distinct ways of creating entanglement is to consider walker systems that carry state. In this context, a walker system is represented by a tripartite system $\mathcal{H}_W = \mathcal{H}_V \otimes \mathcal{H}_C \otimes \mathcal{H}_S$, where $\mathcal{H}_S$ refers to the state carried by the walker. The addition of the state subsystem is interesting to the case of multiple walkers because it enables the generation of an entangled pair between $A$ and $B$ by the 

==> state_walker.tex <==
\section{Walking on the network space} \label{sec:network_state}

The global state of the network is the joint state of all qubits of nodes represented in the Hilbert space $\mathcal{H}^{2^{2m}}$, where $m$ is the number of edges (channels) in the network graph. The fundamental idea explored in this section is to map each state in $\mathcal{H}^{2^{2m}}$ to an edge in a graph and show that the operations used by entanglement routing protocols can be mapped to coin and shift operators in this new graph. 
% The walker model to be describes in this section does not represent a quantum walk on the network graph, instead it walks on $\mathcal{H}^{2m}$. Differently than the walker model presented in Section \ref{sec:assisted}, it servers the single purpose of simulating the behavior of entanglement routing protocols within a quantum walker framework. 

\subsection{State graph}

In order to describe the graph the walker moves on, it is interesting to start with a single edge of the network, which translates to two qubits, and then extrapolating the results to all edges of the network. Let $e = (u, v) \in E$ refer to an edge of the network, with its two qubits being represented by $q_u$ and $q_v$.  It is possible to map the two-qubit computational basis into the edge set of the graph $K_2= (\{0, 1\}, \{(0, 0), (0, 1), (1, 0), (1, 1)\})$, which is a fully-connected 2-vertex graph with self-loops. The choice of a particular mapping between edges and vectors should help describing the generation of a Bell state between $q_u$ and $q_v$ through a quantum walk on $K_2$. Thus, the mapping function
\begin{align}
    & M: (0,0) \to \ket{10}, (0, 1) \to \ket{01}, (1,0) \to \ket{00}, (1,1) \to \ket{11},
\end{align}
which can be visualized in Figure \ref{fig:walk_2graph}(\subref{subfig:k2}), is chosen. Such mapping is of particular interest because it enables describing maximally entangled states by only using edges from a single vertex, shaping the quantum walk dynamics to be described. In particular, we reduce the problem of entanglement generation to the problem of concentration of a quantum walker in a single vertex of the graph.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \input{drawings/k2/k2}
        \caption{Map for $K_2$.}
        \label{subfig:k2}
    \end{subfigure} \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \input{drawings/k2/k2_separable}
        \caption{Separable state.}
        \label{subfig:k2_sep}
    \end{subfigure} \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \input{drawings/k2/k2_coin}
        \caption{State after $C$.}
        \label{subfig:k2_coin}
    \end{subfigure} \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \input{drawings/k2/k2_entangled}
        \caption{EPR pair after $SC$.}
        \label{subfig:k2_ent}
    \end{subfigure} \hfill
    \caption{Quantum walker states on $K_2$ representing one edge of a quantum network. (\subref{subfig:k2}) The edges of a 2-vertex complete graph with self-loops can be used to represent a 2-qubit Hilbert space, were labels show the mapping between edges and vectors. In the context of a quantum walk, the given map enables representing EPR pairs by constructing wavefunctions in which the walker is \textit{vertex-localized}, i.e all the states with non-zero component are edges departing from the same vertex. (\subref{subfig:k2_sep}) A separable state of the $2$-qubits is a \textit{spread} state of the quantum walk, such that one edge of each vertex appears with a non-zero component in the superposition. (\subref{subfig:k2_coin}) Once the coin operator defined in \eqref{eq:coin_k2} is applied, the states have their degree of freedom swapped and (\subref{subfig:k2_ent}) an entangled state is obtained with the application of the the flip-flop operator $S$ defined for $K_2$.}
    \label{fig:walk_2graph}
\end{figure}

We extend this representation to all edges of the network by considering that each edge is represented through a 2-vertex complete graph and taking the graph product between all of them. Such extension is simply visualized by considering two edges and taking the graph product between $K_2$, that represents a single edge, with itself. This results in $K_4$, a 4-vertex complete graph capable of codifying all possible states of $4$-qubits, as shown in Figure \ref{fig:walk_4graph}(\subref{subfig:k4}). Note that GHZ states between the $4$ qubits are still expressed by edges departing from a single vertex, although separable states of EPR pairs are also contemplated by vertex-localized quantum walker states. From now on, we denote $K_T$ as a $T$-vertex complete graph, where labels for vertices follow the graph product between $K_2$. When all $m$ edges of the network are considered, the resulting complete graph has $2^{m}$ nodes and $2^{2m}$ edges, which defines a coined quantum walk space $\mathcal{H}_w = \mathcal{H}^{2^{m}} \otimes \mathcal{H}^{2^{m}}$.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \input{drawings/k4/k4}
        \caption{$K_4$.}
        \label{subfig:k4}
    \end{subfigure} \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \input{drawings/k4/k4_sep}
        \caption{Separable initial state.}
        \label{subfig:k4_sep}
    \end{subfigure} \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \input{drawings/k4/k4_ent}
        \caption{Entangled state after $SC$.}
        \label{subfig:k4_ent}
    \end{subfigure} \hfill
    \caption{Extension for two network edges through graph product. (\subref{subfig:k4}) The product between $K_2$ with itself yields $K_4$, where both vertex and edge labels follow the mapping presented in Figure \ref{subfig:k2}, i.e the vertex $00$ of $K_4$ is obtained by considering two vertices labeled $0$ from $K_2.$ (\subref{subfig:k2_sep}) An initial separable state contains, in this case, $4$ edges. Note that the labels are also simply obtained by looking at the edges of $K_2$. (\subref{subfig:k2_ent}) Again, a single application of the operator $SC$ concentrates the walker function into one vertex, generating a separable state between two EPR pairs.}
    \label{fig:walk_4graph}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \input{drawings/k4/k4_ent}
        \caption{2 entangled pairs.}
        \label{subfig:k41}
    \end{subfigure} \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \input{drawings/k4/k4_c1}
        \caption{After applying $C_{i1}$.}
        \label{subfig:k41_sep}
    \end{subfigure} \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \input{drawings/k4/k4_c2}
        \caption{After applying $C_{i2}$.}
        \label{subfig:k41_ent}
    \end{subfigure} \hfill
    \caption{Extension for two network edges through graph product. (\subref{subfig:k4}) The product between $K_2$ with itself yields $K_4$, where both vertex and edge labels follow the mapping presented in Figure \ref{subfig:k2}, i.e the vertex $00$ of $K_4$ is obtained by considering two vertices labeled $0$ from $K_2.$ (\subref{subfig:k2_sep}) An initial separable state contains, in this case, $4$ edges. Note that the labels are also simply obtained by looking at the edges of $K_2$. (\subref{subfig:k2_ent}) Again, a single application of the operator $SC$ concentrates the walker function into one vertex, generating a separable state between two EPR pairs.}
    \label{fig:walk_4graph_BSM}
\end{figure}

\subsection{Creation of maximally entangled states in network edges}

The first step towards the complete description of a protocol following \eqref{eq:protocol_model} is to show how to generate an EPR pair between the two qubits $q_u$ and $q_v$ of a given edge $e = (u, v)$. The fundamental restriction in this case refers to using the channel to create a maximally entangled state when the initial state of $q_u$ and $q_v$ is separable. The independence of edges enables the description of the process for the case of a single edge and its extension for all edges following a similar approach to the one presented in the previous section. In a nutshell, our goal is to describe coin and shift operators in $K_2$ that evolves a walker state prepared as a separable state of $q_u$ and $q_v$ into an EPR pair.

A simplistic way to generate an EPR pair from a separable state is to prepare $q_u$ and $q_v$ into state
\begin{align}
    \ket{\Psi(0)} = \frac{1}{\sqrt{2}} (\ket{0} + \ket{1}) \otimes \ket{0}  \label{eq:+0},
\end{align}
and then apply a CNOT operator controlled by $q_u$. In terms of the quantum walk in $K_2$, the state described in \eqref{eq:+0} is the state 
\begin{align}
    & \ket{\Phi(0)} = \frac{1}{\sqrt{2}} (\ket{0, 0} + \ket{1, 0})
\end{align}
depicted in Figure \ref{fig:walk_2graph}(\subref{subfig:k2_sep}). Note that $\ket{\Phi(0)}$ is described in terms of the edges of $K_2$ since it is the wavefunction of a quantum walker system. The evolution of the walker must concentrate all of its wavefunction in vertex $1$, since the outcome of the CNOT operator applied in $\ket{\Psi(0)}$ is $(\ket{00} + \ket{11}) / \sqrt{2}$. Considering the flip-flop operator defined for $K_2$ to be the shift operator for the quantum walk, the coin operator
\begin{align}
    & C_2 = I_2 \otimes X, \label{eq:coin_k2}
\end{align}
where $I_2$ is the identity matrix for $\mathcal{H}^2$, is the missing piece needed to generate the entangled state. In this context, a single application of the operator $SC$ generates the state $\ket{\Phi(1)} = (\ket{1, 0} + \ket{1, 1}) / \sqrt{2}$, which is mapped back to the desired EPR pair following the mapping function defined in Figure \ref{fig:walk_2graph}(\subref{subfig:k2}). Note that any of the four Bell states can be obtained in a similar way considering different initial states.

The independence of edges enables a simple construction for the coin operator that simultaneously performs the entanglement generation in all edges of the network. By initially considering the case of 2 network edges, the separable state in which the $4$ qubits are initialized uses the edges of $K_4$ depicted in Figure \ref{fig:walk_4graph}(\subref{subfig:k4_sep}). We refer to the two edges in question to be $e_i = (u_i, v_i)$ for $i \in \{0, 1\}$. The nodes in $K_4$ are labeled following the graph labels for each edge in $K_2$, such that the node $ij \in K_4$ refers to node $i \in K_2$ for $e_0$ and node $j \in K_2$ for $e_1$. The labels in $K_4$ are used to define the coin operator
\begin{align}
    & C_4 = I_4 \otimes X \otimes X
\end{align}
which can simply be written as $C_4 = C_2 \otimes C_2$. The shift operator $S$ is the flip-flop operator in $K_4$ and a single application of $SC_4$ leaves the system in the state $\bigotimes_{i=0}^{1} \ket{00} + \ket{11} / \sqrt{2}$. Thus, for $m$ edges, the coin operator is simply $\bigotimes_{i = 0}^{m}C_2$, which is a separable operator as expected.


\subsection{Entanglement Swapping and GHZ projections}

The separable form obtained is intuitive since we extend the coin operator using edge-independence. Nonetheless, in order to represent generic routing operations, we must be able to write entanglement swapping operations as walks in the complete graph. Since measurements are not unitary, the walker formalism must rely on a stochastic process to recover the behavior of entanglement swapping. This stochastic process chooses coins at random to perform the evolution of the walker, recovering the random nature of projective measurements

Thus, consider the case of a three-node repeater chain, depicted in Figure \ref{subfig:swap_chain}, where each repeater has two quantum memories. By applying the separable generation of EPR pairs in the network edges, the walker state for the product state of the two EPR pairs in edges $(A, u)$ and $(u, B)$ is the uniform superposition of the $4$ edges depicted in Figure \ref{fig:walk_4graph}(\subref{subfig:k4_ent}). To perform entanglement swapping, the two qubits in $u$ are measured together in the Bell basis, with $0.25$ probability of having each one of the Bell states as an output. In the walker representation, we associate each of the Bell states with a set of two coins $\{(C_{i1}, C_{i2})\}$, $i = \{1,...,4\}$, that are applied to the walker wavefunction propelling the one-step evolution
\begin{align}
    & \ket{\Psi(t + 1)} = IC_{i2}C_{i1} \ket{\Psi(t)}, \label{eq:two_step}
\end{align}
where the shift operators is the identity. The first matrix $C_{i1}$ is a permutation of the Hadamard matrix $H$, concentrating the $4$-edge uniform superposition in a single edge, and the stochastic process specifies one between two possible permutations of $H$. The second coin matrix is an extension of a $2$-qubit Hadamard gate to the $4$-qubit space, where the stochastic process defines the extension, and maps a single-edge state into a two-edge uniform superposition. The product $C_{i2}C_{i1}$ is itself a coin operator, since it acts on the subspace of degrees of freedom of the walker, and a single step of evolution suffices to reconstruct a BSM in this formalism.

Furthermore, performing generic GHZ projections is analogous to the BSM case, where differences lay on the dimension of the Hadamard operations and the number of outcomes for the stochastic process. Consider a generalization of a $3$-node repeater chain to a $4$-node star topology shown in Figure \ref{fig:swap}(\subref{subfig:swap_star}), where the center node has $3$-qubits, each of which is entangled to a qubit in the leaves. The six qubit state is represented in $K_8$. The stochastic process to represent a GHZ measurement outputs one of the eight GHZ states with probability $1/8$, which again specifies the set  $\{(C_{i1}, C_{i2})\}$ for $i = \{1,...,8\}$. In this case, $C_{i1}$ is a permutation of $H_8$, the Hadamard operation for the $3$-qubit space, and $C_{i2}$ is an extension of the $1$-qubit Hadamard operation to the $3$-qubit space.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \input{drawings/swapping/chain}
        \caption{Three-node repeater chain.}
        \label{subfig:swap_chain}
    \end{subfigure} \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \input{drawings/swapping/star}
        \caption{Four-node star topology.}
        \label{subfig:swap_star}
    \end{subfigure} \hfill
    \caption{Topology representation for repeater connectivity. GHZ projections are implemented in the quantum walk formalism by a mapping between GHZ states and coin operators in a complete graph. The mapping is a random variable that outputs coin operators uniformly. (\subref{subfig:swap_chain}) To emulate a BSM in a three-node topology, it suffices to sample uniformly from the set $\{0, 1\}^2.$ (\subref{subfig:swap_star}) A GHZ projection in the four-node star is emulated in the complete graph quantum walk framework by sampling uniformly from $\{0, 1\}^3.$}
    \label{fig:swap}
\end{figure}


\subsection{Generalization and reconstruction of protocols}

Essentially, the walker dynamics defined for the complete graph map the problem of entanglement generation in a network to the problem of walker concentration in a graph. The number of edges in the network fix the number of nodes in the complete graph and the graph product operation enables the description of this complete graph based on the mapping between $2$-qubits and $K_2$. In the general case of $m$ edges, coin operators for $K_{2^{m}}$ are constructed in a separable way, following the coin operators defined for $K_2$. Thus, the external phase of entanglement generation protocols, represented in \eqref{eq:protocol_model} by the operator $A(t)$,  is attainable in a single step of the walker, regardless of which one of the four Bell states are shared between the edges. In addition, the stochastic process presented in the previous section allows for the description of $B(t)$ in \eqref{eq:protocol_model} with another step of the walker. Note that the separability in the description of the walker is critical to describe states efficiently, because edges can be analyzed independently when recovering the behavior of both $A(t)$ and $B(t)$.

Following the reconstructions performed for the model presented in Section 3, we now show how to recover the behavior of the BSM protocol defined in \cite{pant2019routing}, assuming global link state knowledge and multi-path routing. The reconstruction is straightforward. Assuming that entanglement generation in each channel of the network succeeds with probability $p$, let $E_P$ be a set of edges chosen at random with probability $p$. For each edge in $E_P$ a walk in $K_2$ is initialized in state \eqref{eq:+0} and an EPR pair is generated following the coin operator in \eqref{eq:coin_k2}. The state of all $|E_P|$ edges is a separable state formed by $|E_P|$ EPR pairs, which is a vertex-localized state in $K_{2^{|E_P|}}$. Finally, considering that an entanglement pair is to be distributed between nodes $A$ and $B$, BSMs are performed by greedily choosing a set of edge-disjoint minimum paths connecting $A$ and $B$ in the subgraph spanned by $E_P$. For each one of this paths, the BSMs will be performed through an stochastic processes defining which coin operators must be applied. In this context, the commutativity between BSMs allow for the construction of a separable coin operator on each pair of qubits operated. In addition, the failure of a BSM operation can be included in the stochastic process defined by adding the identity operator as an output and choosing appropriate probabilities.

The representation of the $4$-GHZ protocol defined in \cite{patil2020entanglement} for the grid follows along the same lines. The external phase is exactly the same, using $E_P$ to select edges. On the other hand, the internal phase is simply obtained by performing $k$-qubits GHZ projections in a node $v$, where $k$ is the degree of $v$ in $E_P$. Since this projections also commute, the only difference lies on the stochastic process and the dimensions of the separable coin operators. Once more, the failure of GHZ projections is incorporated into the stochastic process that select the coins to be applied.
% MORE ON THIS LATER

% It is usually the case that entanglement generation protocols make use of the channels connecting nodes to generate EPR pairs between locally separated qubits. The qubits siting on the channels are, for this matter, independent such that the EPR pair generation on all channels of the network can be performed concurrently. This joint generation is commonly referred as the \textit{external phase} of entanglement generation protocols. Our model

% \subsection{Coin operator}

% The coin operator that performs the walk on $\mathcal{H}^{2m}$ depends on the internal operators of the protocol to be simulated, \textit{i.e} the operators local to qubits in the nodes, which is defined by the operator $A(t)$ in \eqref{eq:protocol_model}. The locality of operations in the nodes is captured by considering that each node applies a local unitary operator on its memories and constructing a separable global coin operator from them. To establish nomenclature, consider that a \textit{step} of the protocol is defined as any set of operations that can be done concurrently and a \textit{round} to be one complete execution of a protocol, i.e the sequence of steps needed to perform a given global operation on the network memories. Let $C_v(t)$ be the local operator applied by node $v$ at time $t$ on its memories. The global coin operator is the separable operator
% \begin{align}
%     & C(t) = \bigotimes_{v} C_v(t), \label{eq:global_coin_op}
% \end{align}
% where $t$ is discrete and describes a step of the protocol. To give examples, if $C_v$ is a CNOT operation on all qubits of $v$, full GHZ states can be generated in each step of the protocol, if $C_v$ is a pairwise CNOT gate, entanglement pairs can be generated throughout the qubits of a node at each coin flip.

% \subsection{Shift operator}

% The shift operator depends on the external phase of the protocol to be simulated and eventually needs to account for transmission effects and the analysis presented here is an initial effort. Again, recall that all operations considered are assumed to be unitary. In quantum walks, shift operators are permutations of the basis vectors of the walker space, which are edges of the graph. This implies that a process can be described as a walk if it can be decomposed into a coin operator followed by a permutation of the basis states. Thus, let $S_{uv}(t)$ denote the operator that acts on the memories incident to the edge (channel) $(u, v)$ of the network graph at step $t$. Since edge operations are all separable, the global operator is
% \begin{align}
%     & S(t) = \bigotimes_{(u, v) \in E, u < v} S_{uv}(t).
% \end{align}
% $S(t)$ is a valid shift only if it can be written as a permutation operator on the space $\mathcal{H}^{2^{m}}$. A sufficient condition for $S(t)$ to be a permutation operator is to have $S_{uv}$ be a permutation operator on the space of the edge qubits $(u, v)$. Interestingly, this is sufficient to capture the external phase of entanglement routing protocols, which happens to be the case because the CNOT operator is a permutation operator. Consider a single pair of nodes $u, v$ in the network and the edge connecting them. Let the edge swap operator
% \begin{align}
%     & S_{uv}(t) = \dyad{0} \otimes I + \dyad{1} \otimes X 
%     % & S: \ket{00} \rightarrow \ket{00}; \ket{01} \rightarrow \ket{01} ; \ket{10} \rightarrow \ket{11} ; \ket{11} \rightarrow \ket{10}.
% \end{align}
% be defined as the CNOT operator. Note that $S_{uv}(t)$ satisfies the following permutation rules
% \begin{align}
%     & S_{uv}(t): \ket{00} \rightarrow \ket{00}; \ket{01} \rightarrow \ket{01} ; \ket{10} \rightarrow \ket{11} ; \ket{11} \rightarrow \ket{10}.
% \end{align}

% \subsection{Simulating entanglement routing protocols}

% The quantum walk formalism demands that every step of the walker dynamics start with a coin flip. To recover the external phase of entanglement routing protocols, the first coin flip is used to prepare the state of network memories to generate entanglement between edges when the first shift operator is applied. The external phase is trivially recovered by applying the coin operator followed by an identity shift. Thus,
% assuming that the network state can be prepared as the separable state $\ket{\Psi(0)} = \ket{0,\ldots, 0}$, the first coin operator of vertex $u$ is
% \begin{align}
%     & C_u(0) = \bigotimes_{u \in \delta(v)} \mathbbm{1}_{u > v} I + \mathbbm{1}_{u < v} H,
% \end{align}
% where $\mathbbm{1}$ is the Kronecker delta function, $I$ is the identity and $H$ is the Hadamard operator. Note that the selection rule for the delta function ensures that only a single qubit of each edge of the graph goes through a Hadamard operator when the global coin operator defined in \eqref{eq:global_coin_op} is applied to the network. To ensure the correct application of coin operators by vertices, we assume that the qubits in the network state are in lexical order of edges. To verify that entangled pairs are generated on each edge of the network, it is enough to analyze the behavior of a single edge due to the separability of $S(t)$. Hence, let vector $\ket{q_{uv}}$ represent the qubit of $u$ that is incident to edge $(u, v)$, for every edge $(u, v) \in E$. Considering edge $(u, v)$, with $u < v$ yields
% \begin{align}
%     & S_{uv}(0)(C_u(0)\otimes C_v(0))\ket{\Psi(0)} = S(0) \frac{1}{\sqrt{2}} (\ket{0_{uv}0_{vu}} + \ket{1_{uv}0_{vu}}), \\
%     & S_{uv}(0)(C_u(0)\otimes C_v(0))\ket{\Psi(0)} = \frac{1}{\sqrt{2}} (\ket{0_{uv}0_{vu}} + \ket{1_{uv}1_{vu}}). \label{eq:edge_entanglement}
% \end{align}







% To simulate the entanglement routing protocol described in \cite{pant2019routing}, let the coin operator for the external phase recovery to be defined as a CNOT between two qubits 

% Assume that $u$ and $v$ each have $4$ memory qubits denoted as $\ket{u_0u_1 u_2 u_3}$ and $\ket{v_0v_1 v_3 v_3}$. Assume that the network initial state is $\ket{\Psi(0)} = \ket{0000} \otimes \ket{0000}$. Let $C_v$ be an operator that entangles the first and second pairs of qubits together. $C$ and $S$ yield
% \begin{align}
%     & \ket{\Psi(0)} = \ket{0000} \otimes \ket{0000} \\
%     & C \ket{\Psi(0)} = \frac{1}{\sqrt{2}} (\ket{00} + \ket{11}) \otimes \frac{1}{\sqrt{2}} (\ket{00} + \ket{11}) \otimes \frac{1}{\sqrt{2}} (\ket{00} + \ket{11}) \otimes \frac{1}{\sqrt{2}} (\ket{00} + \ket{11}) \\
%     & SC \ket{\Psi(0)} = \frac{1}{\sqrt{2}} (\ket{0_{u_0} 0_{v_0}} + \ket{1_{u_0} 1_{v_0}}) \otimes \frac{1}{\sqrt{2}} (\ket{0_{u_1} 0_{v_1}} + \ket{1_{u_1} 1_{v_1}}) \ldots
% \end{align}
% Note that $S$ swapped the entanglement between pairs $u_0u_1$ and $v_0v_1$. If $C_v$ performs mutlipartite entanglement on all nodes, this simple scheme recovers the GHZ protocol.

% \subsection{Discussion}

% To extend the framework to generic protocols represented in the LOCC formalis, it is necessary to show that $S$ can always be made a permutation operator. Nonetheless, some important considerations follows. If $S(t)$ and $C(t)$ commutes for all $t$ then the final state of the network after a round of the protocol with $t$ steps is
% \begin{align}
%     & \ket{\Psi(t)} = \prod_{k = 0}^{t}S(k) \prod_{k = 0}^{t}C(k) \ket{\Psi(0)}
% \end{align}
% This implies that any sort of protocol can be implemented in a single round. In addition, since $C_v$ and $S_{uv}$ are separable operators, $C$ and $S$ can be simply diagonalized through the separate diagonalization of $C_v$ and $S_{uv}$, for all vertex $v$ and edge $(u, v)$ respectively. This spectral decomposition can be interesting to the analysis of protocols since it simplifies many calculations.

% \subsection{Representing GHZ protocols}

% \begin{align}
%     & \ket{\Psi(0)} = \ket{0} \\
%     & C_v(0) = (\dyad{0} \otimes I + \dyad{1} \otimes X) H \otimes I \\
%     & C_v(0) = \dyad{0}H \otimes I + \dyad{1}H \otimes X
    
%     & S_{e}(0): \ket{00} \rightarrow \ket{00}; \ket{01} \rightarrow \ket{10} ; \ket{10} \rightarrow \ket{01} ; \ket{11} \rightarrow \ket{11} \\
%     & 
% \end{align}


